Logic-Based Explainability in Machine Learning

The last decade witnessed an ever-increasing stream of successes in Machine Learning (ML). These successes offer clear evidence that ML is bound to become pervasive in a wide range of practical uses, including many that directly affect humans. Unfortunately, the operation of the most successful ML models is incomprehensible for human decision makers. As a result, the use of ML models, especially in high-risk and safety-critical settings is not without concern. In recent years, there have been efforts on devising approaches for explaining ML models. Most of these efforts have focused on so-called model-agnostic approaches. However, all model-agnostic and related approaches offer no guarantees of rigor, hence being referred to as non-formal. For example, such non-formal explanations can be consistent with different predictions, which renders them useless in practice. This paper overviews the ongoing research efforts on computing rigorous model-based explanations of ML models; these being referred to as formal explanations. These efforts encompass a variety of topics, that include the actual definitions of explanations, the characterization of the complexity of computing explanations, the currently best logical encodings for reasoning about different ML models, and also how to make explanations interpretable for human decision makers, among others.

==> runex/runex01b.tex <==

\begin{example} \label{ex:runex02}
  The second running example is a decision list, and it adapted
  from~\cite{rivest-ml87}
  %~\cite{ims-sat21}.
  %
  %Concretely, $\fml{F}=\{1,2\}$, $\fml{D}_1=\fml{D}_2=\{0,1\}$,
  %$\fml{K}=\{0,1\}$, and $\kappa$ is defined by~\cref{fig:runex02}.
  %Furthermore, the instance is $(\mbf{v},c)=((0,1),1)$.
  Concretely, $\fml{F}=\{1,2,3,4,5\}$,
  $\fml{D}_i=\{0,1\},i=1,\ldots,5$,
  $\fml{K}=\{0,1\}$, and $\kappa$ is defined by~\cref{fig:runex02}.
  Furthermore, the instance is $(\mbf{v},c)=((1,0,1,0,1),0)$.
\end{example}
%
\begin{figure}[t]
  \begin{center}
    %\renewcommand{\arraystretch}{1.35}
    %\begin{tabular}{|c|} \hline
    \boxedeq{eq:fig}{
      \renewcommand{\arraystretch}{1.15}
      \begin{array}{lllcl}
        \tn{R$_{0}$:} & \tn{IF~}      & (x_1\land\neg{x_3}) & \tn{~THEN~} & 0 \\
        \tn{R$_{1}$:} & \tn{ELSE IF~} & (\neg{x_1}\land{x_2}\land{x_5}) & \tn{~THEN~} & 1 \\
        \tn{R$_{2}$:} & \tn{ELSE IF~} & (\neg{x_3}\land\neg{x_4}) & \tn{~THEN~} & 1 \\
        \tn{R$_{\tn{\sc{def}}}$:} & \tn{ELSE~} & \quad\quad & \tn{~THEN~} & 0 %\\
      \end{array}
    }
    %  \\ \hline
    %\end{tabular}
  \end{center}
  \caption{Decision list running example} \label{fig:runex02}
\end{figure}


\begin{comment}
\begin{figure}[t]
  \begin{center}
    %\renewcommand{\arraystretch}{1.35}
    %\begin{tabular}{|c|} \hline
    \boxedeq{eq:fig}{
      \renewcommand{\arraystretch}{1.15}
      \begin{array}{lllcl}
        \tn{R$_{0}$:} & \tn{IF~}      & x_1 & \tn{~THEN~} & 1 \\
        \tn{R$_{1}$:} & \tn{ELSE IF~} & x_2 & \tn{~THEN~} & 1 \\
        \tn{R$_{\tn{\sc{def}}}$:} & \tn{ELSE~} & \quad\quad & \tn{~THEN~} & 0 %\\
      \end{array}
    }
    %  \\ \hline
    %\end{tabular}
  \end{center}
  \caption{Decision list running example} \label{fig:runex02}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[t]
  \begin{center}
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{ccc|ccc} \hline
      \quad\quad & Decision List & \quad\quad\quad &
      \quad\quad\quad & Additional detail & \quad\quad \\ \hline
      &
      $
      \begin{array}{lllcl}
        \tn{R$_{0}$:} & \tn{IF~}      & x_1 & \tn{~THEN~} & 1 \\
        \tn{R$_{1}$:} & \tn{ELSE IF~} & x_2 & \tn{~THEN~} & 1 \\
        \tn{R$_{\tn{\sc{def}}}$:} & \tn{ELSE~} & \quad\quad & \tn{~THEN~} & 0 \\
      \end{array}
      $
      & \quad\quad & \quad\quad &
      $
      \begin{array}{ccc}
        \fml{F} & = & \{1,2\} \\
        \fml{D}_1,\fml{D}_2 & = & \{0,1\} \\
        \fml{K} & = & \{0,1\} \\
      \end{array}
      $
      &
      \\ \hline
    \end{tabular}
  \end{center}
  \caption{Decision list running example} \label{fig:runex02}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[t]
  \begin{subfigure}[b]{0.5\textwidth}
    \boxedeq{def:runex02a}{
      %\[
      \begin{array}{lllcl}
        \tn{R$_{0}$:} & \tn{IF~}      & x_1 & \tn{~THEN~} & 1 \\[2pt]
        \tn{R$_{1}$:} & \tn{ELSE IF~} & x_2 & \tn{~THEN~} & 1 \\[2pt]
        \tn{R$_{\tn{\sc{def}}}$:} & \tn{ELSE~} & \quad\quad & \tn{~THEN~} & 0 \\
      \end{array}
      %\]
    }
    \caption{Decision list}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.5\textwidth}
    \vspace*{-50pt}
    \boxedeq{def:runex02b}{
      \begin{array}{ccc}
        \fml{F} & = & \{1,2\} \\[2pt]
        \fml{D}_1,\fml{D}_2 & = & \{0,1\} \\[2pt]
        \fml{K} & = & \{0,1\} \\
      \end{array}
    }
    \caption{Additional detail}
  \end{subfigure}
  \caption{Decision list running example} \label{fig:runex02}
\end{figure}
\end{comment}


==> texfigs/exnn01.tex <==
\tikzset{basic/.style={draw,fill=none,
  text badly centered,minimum width=3em}}
\tikzset{input/.style={basic,circle,minimum width=3.5em}}
\tikzset{weights/.style={basic,rectangle,minimum width=2em}}
\tikzset{functions/.style={basic,circle, minimum width=4em}}
\newcommand{\addaxes}{\draw (0em,1em) -- (0em,-1em)
  (-1em,0em) -- (1em,0em);}
\newcommand{\relu}{\draw[line width=1.5pt] (-1em,0) -- (0,0)
  (0,0) -- (0.75em,0.75em);}
\newcommand{\stepfunc}{\draw[line width=1.5pt] (0.65em,0.65em) -- (0,0.65em) 
  -- (0,-0.65em) --
  (-0.65em,-0.65em);}

\begin{tikzpicture}[scale=1.2]
  % Draw input nodes
  \node[input] (f0) at (0,1.5cm) {$x_0=1$};
  \node[input] (f1) at (0,0cm) {$x_1$};
  \node[input] (f2) at (0,-1.5 cm) {$x_2$};
  % Draw summation node
  \node[functions] (sum) at (2,0) {\Huge$\sum$};
  \node[above=0.70cm] at (sum) {Sum};
  \node[below=0.69cm,xshift=0.225cm] at (sum) {$y_1=\sum_{i=0}^n w_ix_i$};
  % Draw node for activation function
  \node[functions] (activation) at (4,0) {};
  % Place activation function in its node
  \begin{scope}[xshift=4cm,scale=1.25]
    \addaxes
    % flexible selection of activation function
    \relu
    % \stepfunc
  \end{scope}
  % Connect sum to relu
  \draw[->] (sum) -- (activation);
  \draw[->] (activation) -- ++(1,0);
  % Edges
  \draw[->] (f0) -- (sum);
  \draw[->] (f1) -- (sum);
  \draw[->] (f2) -- (sum);
  %
  \node at (0.525cm,0.8cm) {-0.5};
  \node at (1.12cm,0.175cm) {+1};
  \node at (0.525cm,-0.8575cm) {+1};
  % Labels
  %\node[above=0.625cm] at (f0) {Inputs};
  \node[below left=0.275cm and -0.575cm of f1] {Inputs};
  \node[above=0.7cm] at (activation) {ReLU};
  \node[below=0.7125cm,xshift=0.225cm] at (activation) {$t_1=\max(y_1,0)$};
  %
  \node[above right=-0.4cm and 0.2cm of sum] {$y_1$};
  \node[above right=-0.4cm and 0.2cm of activation] {$t_1$};
  %
  % Expressions
  \node[below right=1cm and 0.125cm of sum] {$\begin{array}{l}t_1=\max(x_1+x_2-0.5,0)\\o_1=\tn{ITE}(t_1>0,1,0)\\\end{array}$};
\end{tikzpicture}


==> texfigs/tree04b.tex <==
% Example from Rudin et al. NeurIPS'19 paper
%%
%\tikzset{every label/.style={xshift=-0.35ex,
%  yshift=-5.25ex,
%  text width=1ex,
%  align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%
%\tikzset{tlabel/.style={xshift=0.25ex, yshift=1.75ex, text width=1ex,
%    align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%%\tikzset{every node/.style={---rectangle---}}
%
\forestset{
  BDT/.style={
    for tree={
      l=1.5cm,s sep=1.15cm,
      if n children=0{}{circle}, %rectangle
      %if n children=0{}{draw},
      draw=black,%draw=midblue,
      text=black,%text=midblue,
      edge={
        my edge
      },
      if n=1{
        edge+={0 my edge},
      }{},
      edge=thick,
      %font=\sffamily,
    }
  },
}
%
% middle-middle=x : x_1
% top-left=x : x_2
% bottom-right=x : x_3
% bottom-left=x : x_4
% top-right=x : x_5
%
\begin{forest}
  BDT
  [{$x_1$}, label={[yshift=-6.875ex]{{\tiny1}}} %middle-middle=x
    [{$x_2$}, label={[yshift=-6.875ex]{{\tiny2}}}, %top-left=x
      edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}}
      [{$x_3$}, label={[yshift=-6.875ex]{{\tiny4}}}, %bottom-right=x
        edge label={node[midway,left,xshift=-2.5pt] {{\scriptsize$\in\{0\}$}}}
        [\rhlight{\textbf{0}}, label={[yshift=-5.0ex]{{\tiny6}}},
          edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}},
          rectangle, fill={tred3!20} ]
        [{$x_4$}, label={[yshift=-6.875ex]{{\tiny7}}}, %bottom-left=x
          edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}}
          [{$x_5$}, label={[yshift=-6.875ex]{{\tiny10}}}, %top-right=x
            edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
            [\rhlight{\textbf{0}}, label={[yshift=-5.0ex]{{\tiny14}}},
              edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}},
              rectangle, fill={tred3!20} ]
            [\dghlight{\textbf{1}}, label={[yshift=-5.0ex]{{\tiny15}}},
              edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
              rectangle, fill={tgreen3!25} ]
          ]
          [\dghlight{\textbf{1}}, label={[yshift=-5.0ex]{{\tiny11}}},
            edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
            rectangle, fill={tgreen3!25} ]
        ]
      ]
      [{$x_4$}, label={[yshift=-6.875ex]{{\tiny5}}}, %bottom-left=x
        edge label={node[midway,right,xshift=1.5pt] {{\scriptsize$\in\{1\}$}}}
        [{$x_5$}, label={[yshift=-6.875ex]{{\tiny8}}}, %top-right=x
          edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}}
          [\rhlight{\textbf{0}}, label={[yshift=-5.0ex]{{\tiny12}}},
            edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}},
            rectangle, fill={tred3!20} ]
          [\dghlight{\textbf{1}}, label={[yshift=-5.0ex]{{\tiny13}}},
            edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
            rectangle, fill={tgreen3!25} ]
        ]
        [\dghlight{\textbf{1}}, label={[yshift=-5.0ex]{{\tiny9}}},
          edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
          rectangle, fill={tgreen3!25} ]
      ]
    ]
    [\dghlight{\textbf{1}}, label={[yshift=-5.0ex]{{\tiny3}}},
      edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
      rectangle, fill={tgreen3!25} ]
  ]
\end{forest}


==> tikzlibrarytimeline.code.tex <==
% * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
% COPYRIGHT 2014 - Claudio Fiandrino
% Released under the LaTeX Project Public License v1.3c or later
% 
% email: <claudio dot fiandrino at gmail dot com>
%
% Timeline TikZ library version 0.3b - 25/02/2019

\usetikzlibrary{backgrounds,calc}

\pgfkeys{/tikz/.cd,
  timespan/.store in=\timespan,
  timespan=Week,
  timeline width/.store in=\timelinewidth,
  timeline width=20,
  timeline height/.store in=\timelineheight,
  timeline height=1,
  timeline offset/.store in=\timelineoffset,
  timeline offset=0.15,
  initial week/.store in=\initialweek,
  initial week=1,
  end week/.store in=\endweek,
  end week=2,
  time point/.store in=\timepoint,
  time point=0.5,
  between day/.style args={#1 and #2 in #3}{% auxiliary style for days
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between week/.style args={#1 and #2 in #3}{% style for weeks
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between month/.style args={#1 and #2 in #3}{% auxiliary style for months
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between year/.style args={#1 and #2 in #3}{% auxiliary style for years
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  involvement degree/.store in=\involvdegree,
  involvement degree=2cm,
  phase color/.store in=\phasecol,
  phase color=red!50!orange,
  phase appearance/.style={
    circle,
    opacity=0.3,
    minimum size=\involvdegree,
    fill=\phasecol
  },
}
% settings to customize aspect of timeline
\newif\ifcustominterval
\pgfkeys{/tikz/timeline/.cd,
  custom interval/.is if=custominterval,
  custom interval=false,
}

% settings to deploy milestones
\pgfkeys{/tikz/milestone/.cd,
  at/.store in=\msstartpoint,
  at=phase-1.north,
  circle radius/.store in=\milestonecircleradius,
  circle radius=0.1cm,
  direction/.store in=\msdirection,
  direction=90:2cm,
  text/.store in=\mstext,
  text={},
  text options/.code={\tikzset{#1}},
}

\newcommand{\reftimespan}{\MakeLowerCase{\timespan}}

\newcommand{\timeline}[2][]{
  \pgfkeys{/tikz/timeline/.cd,#1}
  \draw[fill,opacity=0.8] (0,0) rectangle (\timelinewidth,\timelineheight);
  \shade[top color=black, bottom color=white,middle color=black!20]
    (0,0) rectangle (\timelinewidth,-\timelineoffset);
  \shade[top color=white, bottom color=black,middle color=black!20]  
    (0,\timelineheight) rectangle (\timelinewidth,\timelineheight+\timelineoffset);

  \ifcustominterval%
    \foreach \smitem [count=\tlmxi] in {#2}  {\global\let\maxsmitem\tlmxi}%
  \else%
    \foreach \smitem [count=\tlmxi] in {1,...,#2}  {\global\let\maxsmitem\tlmxi}%
  \fi%
  
  \pgfmathsetmacro\position{\timelinewidth/(\maxsmitem+1)}
  \node at (0,0.5\timelineheight)(\timespan-0){\phantom{Week 0}};
 
  \ifcustominterval%
    \foreach \x[count=\tlmxi] in {#2}{%
      \node[text=white,text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \else%
    \foreach \x[count=\tlmxi] in {1,...,#2}{%
      \node[text=white, text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \fi%  
}

\newcounter{involv}
\setcounter{involv}{0}

\newcommand{\phase}[1]{
\stepcounter{involv}
\node[phase appearance,#1] 
 (phase-\theinvolv)
 at ($(\timespan-\initialweek)!\timepoint!(\timespan-\endweek)$){};
}

\newcommand{\initialphase}[1]{
\node[phase appearance,#1,anchor=west,between week=0 and 1 in 0,] 
 (phase-\theinvolv)
 at ($(\timespan-0)!0!(\timespan-1)$){};
\setcounter{involv}{0} 
}

\newenvironment{phases}{\begin{pgfonlayer}{background}}{\end{pgfonlayer}}

\newcommand{\addmilestone}[1]{
\pgfkeys{/tikz/milestone/.cd,#1}
\draw[double,fill] (\msstartpoint) circle [radius=\milestonecircleradius];
\draw(\msstartpoint)--++(\msdirection)node[/tikz/milestone/text options]{\mstext};
}

% HISTORY
% 0.1 -> initial release
% 0.2 -> customizable timespan label
% 0.3 -> \timeline command with custom intervals
%             styles ``between x''
%             removed unnecessary call to xstring
% 0.3a -> text depth for timeline labels
% 0.3b -> \xi conflict - thanks Enrico Gregorio (egreg) https://tex.stackexchange.com/q/476089

